Blink: Fast and Generic Collectives for Distributed ML

Model parameter synchronization across GPUs introduces high overheads for data-parallel training at scale. Existing parameter synchronization protocols cannot effectively leverage available network resources in the face of ever increasing hardware heterogeneity. To address this, we propose Blink, a collective communication library that dynamically generates optimal communication primitives by packing spanning trees. We propose techniques to minimize the number of trees generated and extend Blink to leverage heterogeneous communication channels for faster data transfers. Evaluations show that compared to the state-of-the-art (NCCL), Blink can achieve up to 8x faster model synchronization, and reduce end-to-end training time for image classification tasks by up to 40%.

==> listing_macros.tex <==
\usepackage{listings}
% we could try "minted" for highlighting

\definecolor{mygreen}{rgb}{0,0.6,0}
\definecolor{mygray}{rgb}{0.5,0.5,0.5}
\definecolor{mymauve}{rgb}{0.58,0,0.82}

\lstdefinestyle{MyCodeStyle}
%\lstset{ %
{
backgroundcolor=\color{white},   % choose the background color; you must add \usepackage{color} or \usepackage{xcolor}
  basicstyle=\footnotesize,        % the size of the fonts that are used for the code
  breakatwhitespace=true,         % sets if automatic breaks should only happen at whitespace
  breaklines=true,                 % sets automatic line breaking
  captionpos=b,                    % sets the caption-position to bottom
  commentstyle=\color{mygreen},    % comment style
  %deletekeywords={...},            % if you want to delete keywords from the given language
  escapeinside={!}{!},          % if you want to add LaTeX within your code
  extendedchars=true,              % lets you use non-ASCII characters; for 8-bits encodings only, does not work with UTF-8
  %frame=single,                    % adds a frame around the code
  keepspaces=true,                 % keeps spaces in text, useful for keeping indentation of code (possibly needs columns=flexible)
  keywordstyle=\color{blue},       % keyword style
  morekeywords={function,local},            % if you want to add more keywords to the set
  numbers=left,
  numberstyle=\footnotesize\color{mygray},
  xleftmargin=1.8em,
  numbersep=0.8em,
  aboveskip=0pt,
  belowskip=0pt,
  rulecolor=\color{black},         % if not set, the frame-color may be changed on line-breaks within not-black text (e.g. comments (green here))
  showspaces=false,                % show spaces everywhere adding particular underscores; it overrides 'showstringspaces'
  showstringspaces=false,          % underline spaces within strings only
  showtabs=false,                  % show tabs within strings adding particular underscores
  stringstyle=\color{mymauve},     % string literal style
  tabsize=2,                       % sets default tabsize to 2 spaces
  title=\lstname,                   % show the filename of files included with \lstinputlisting; also try caption instead of title
  basicstyle=\ttfamily,
  columns=flexible
}

\lstset{
language=C,                 % the language of the code
}

\usepackage{silence}
\WarningFilter{latex}{Text page iii contains only floats}


%%%%%%%%%%%%%%%
% listing syntax for ModP
%%%%%%%%%%%%%%%
% Define Language
\lstloadlanguages{[Visual]C++}
\lstdefinelanguage{modp}
{
  % list of keywords
  morekeywords={
    module,
    machine,
    refines,
    satisfies,
    test,
    hide,
    in,
    sends,
    send,
    creates,
    private,
    receives, 
    implementation,
    specification, 
    event, 
    model, 
    \$,
    bool,
    any, 
    static, 
    fun, 
    if, 
    int, 
    interface,
    entry,
    state, 
    var,
    new,
    goto,
    hot,
    start,
    on,
    monitor,
    observes,
    eventset, 
    is
  },
  sensitive=false, % keywords are not case-sensitive
  morecomment=[l]{//}, % l is for line comment
  morecomment=[s]{/*}{*/}, % s is for start and end delimiter
  morestring=[b]" % defines that strings are enclosed in double quotes
}

\definecolor{eclipseBlue}{RGB}{42,0.0,255}
\definecolor{eclipseGreen}{RGB}{0, 139, 69}
\definecolor{eclipsePurple}{RGB}{127,0,85}

\lstdefinestyle{ModPCodeStyle}
{
  basicstyle=\ttfamily\footnotesize, % Global Code Style
  captionpos=b, % Position of the Caption (t for top, b for bottom)
  extendedchars=true, % Allows 256 instead of 128 ASCII characters
  tabsize=2, % number of spaces indented when discovering a tab
  columns=fixed, % make all characters equal width
  keepspaces=true, % does not ignore spaces to fit width, convert tabs to spaces
  showstringspaces=false, % lets spaces in strings appear as real spaces
  breaklines=true, % wrap lines if they don't fit
  numbers=left,
  xleftmargin=1.8em,
  numbersep=0.8em,
  aboveskip=0pt,
  belowskip=0pt,
  %frame=tb, % draw a frame at the top, right, left and bottom of the listing
  %frameround=tttt, % make the frame round at all four corners
  %framesep=4pt, % quarter circle size of the round corners
  %numbers=right, % show line numbers at the left
  %numberstyle=\tiny\ttfamily, % style of the line numbers
  commentstyle=\color{eclipseBlue}, % style of comments
  keywordstyle=\bf\color{eclipsePurple}, % style of keywords
  stringstyle=\color{eclipseBlue}, % style of strings
}

\lstset{
language=modp,                 % the language of the code
}


==> tex/approach.tex <==
\section{Approach}
\label{sec:approach}

%NOTE: Cross machine communication can be completely overlap with in-machine GPU communication. It is because cross machine and in-machine communication are using different channels. Cross machine uses PCIe+IB, whereas in machine using NVLink (NV1 or NV2).

\begin{figure*}[t!]
  \centerline{\includegraphics[width=0.95\textwidth]{figs/blink-workflow.pdf}}
  \caption{\system{} Toolchain workflow}
  \label{fig:workflow}
\end{figure*}

\gw{first draft here, may need re-write}

As shown in Figure~\ref{fig:workflow}, {\tt\system{}} first automatically probes the whole system topology. When receiving meta-data of assigned GPUs from resource scheduler, {\tt\system{}} launches Tree Generator (TreeGen) \textbf{XXX: what is filter in mwu?}. Based on assigned GPU group and  its corresponding topology, treeGen outputs maximum number of spanning trees within the topology of allocated GPU group. 

After TreeGen passing the network scheduling results (spanning trees) to our Code Generator (CodeGen), CodeGen automatically generate CUDA code for the implementation of {\tt \system{}}'s collective communication primitives based on the treeGen outputs. It is worth mentioning that, the generated data transfer code exposes exactly the same API as NVIDIA NCCL~\cite{nccl}, and use it to generate our blink library binaries (i.e. libBlink.so).

To seamlessly replace the corresponding NCCL function call, we use \emph{LD\_PRELOAD} trick, which forces our blink library to loaded before NCCL counterpart during dynamic linking process to generate the executable binary for the main program. 

After the whole process mentioned above, the use code (Main Program) can repeatedly make function call to our blink library.

==> tex/eg_code.tex <==
%!TEX root = paper.tex

\section{Code Examples}
\label{sec:code_eg}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Listing 1
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{figure}
  \footnotesize
  \lstinputlisting[language=modp, style=ModPCodeStyle]{./code/pseudocode.p}
  \caption{Pseudocode for SMR linearizability abstraction}
  \label{fig:linearabs}
\end{figure}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Listing 2
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\ctextbf}[1]{\textrm{\textbf{#1}}}

\begin{figure}
\footnotesize
\begin{lstlisting}[style=MyCodeStyle]
// @param  L     maximum level
// @param  wal   write-ahead log file size
// @param  c0    level-0 SSTable count
// @param  size  level sizes
// @return       write amplification
function estimateWA_LevelDB(L, wal, c0, size[]) {
  local l, WA, interval[], write[];

  // mem -> log
  WA = 1;

  // mem -> level-0
  WA += !\ctextbf{unique}!(wal) / wal;

  // level-0 -> level-1
  interval[0] = wal * c0;
  write[1] = !\ctextbf{merge}!(!\ctextbf{unique}!(interval[0]), size[1]);
  WA += write[1] / interval[0];

  // level-l -> level-(l+1)
  for (l = 1; l < L; l++) {
    interval[l] = interval[l-1] + !\ctextbf{dinterval}!(size, l);
    write[l+1] = !\ctextbf{merge}!(!\ctextbf{unique}!(interval[l]), size[l+1]) + !\ctextbf{unique}!(interval[l]);
    WA += write[l+1] / interval[l];
  }

  return WA;
}
\end{lstlisting}\vspace{-2.0em}
% we use figure + captionof to use the same style for both figure/algorithm
%\captionof{algorithm}{Pseudocode of a model of WA of LevelDB\@.}
\caption{Pseudocode of a model of WA of LevelDB\@.}
\label{alg:leveldb}
\end{figure}


==> tex/eg_fig.tex <==
\section{Figures}
\label{sec:figs}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Figure
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\begin{figure}
%  \centerline{\placeholder{Descriptive figure text goes here.}}
%\caption{A placeholder caption for a placeholder figure \boldmath$F$.}
%\label{fig:placeholder}
%\end{figure}

\begin{figure}[t!]
  \centerline{\includegraphics[width=0.95\columnwidth]{figs/topo-dgx.pdf}}
  \caption{Network Topology of DGX-1's 8 GPUs interconnects with NVLink}
  \label{fig:dgx1-topo}
\end{figure}


==> tex/eg_table.tex <==
\section{Tables}
\label{sec:tab}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Tables
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%% http://en.wikibooks.org/wiki/LaTeX/Tables#The_tabular_environment

\newcolumntype{C}{>{\centering\arraybackslash}p{12mm}}
%\newcolumntype{C}{>{\centering}p{12mm}@{}}  % use \tabularnewline instead of \\ in tables

\begin{center}
\begin{tabular}{|C|c|C|C|}
\hline%
1A &\multirow{2}{12mm}{\centering W} & 1 & 2 \\
\cline{1-1} \cline{3-4}%
1B&                                  & 3 & 4 \\
\hline%
2A &\multirow{2}{12mm}{\centering Y} & 5 & 6 \\
\cline{1-1} \cline{3-4}%
2B &                                 & 7 & 8 \\
\hline%
\end{tabular}
\end{center}




\begin{comment}
%\usepackage{multicol}  % causes problem with paper title when in two-column mode

\begin{center}
%\begin{tabular}{|m{0.1\columnwidth}|m{0.2\columnwidth}|m{0.1\columnwidth}|m{0.35\columnwidth}|} 
\begin{tabular}{|l|l|l|l|} 
\hline
Index & \multicolumn{3}{|c|}{Schedulers} \\
\hline
\multirow{3}{*}{1} & \multirow{3}{*}{Immediate}    & RR & Round Robin \\
\cline{3-4}%
                   &                               & EF & Earliest First \\
\cline{3-4}%
                   &                               & LL & Lightest Loaded \\
\hline
\multirow{5}{*}{2} & \multirow{5}{*}{Batch}        & MM & Min-Min \\ 
\cline{3-4}%
                   &                               & MX & Max-Min \\
\cline{3-4}%
                   &                               & DL & Dynamic Level \\ 
\cline{3-4}%
                   &                               & RC & Relative Cost \\
\cline{3-4}%
                   &                               & \multicolumn{2}{c|}{YAY} \\
\hline
\multirow{4}{*}{3} & \multirow{4}{*}{Evolutionary} & PN & This paper \\
                   &                               & ZO & Genetic Algorithm\\
                   &                               & TA & Tabu search\\
                   &                               & SA & Simlulated Annealing \\
\hline
\end{tabular}
\end{center}

\end{comment}



\begin{table*}
\centering
\scriptsize
\begin{tabular}{p{0.12\textwidth}|p{0.28\textwidth}|p{0.5\textwidth}}
Protocol & Safety Spec & Liveness Spec (for $\leq N$ failures)\\
\hline
Two Phase Commit & \textit{Atomicity} & Coordinator makes progress\\\hline
Chain Repl. & All invariants in~\cite{Renesse:osdi2004}, cmd-log consistency &  With stable head node, every cmd is eventually responded to\\\hline
Multi-Paxos & Consensus requirements \cite{Lamport:paxos-simple}, log consistency~\cite{VanRenesse:2015} & For a live quorum of replicas with all nodes trusting the leader has not failed, if the network is eventually synchronous, every proposal is eventually chosen.
%With stable leader, every proposal is always eventually learnt by learners\\\hline
%Basic Paxos & All consensus requirements in \cite{Lamport:paxos-simple} & With distinguished proposer, a proposal is eventually chosen \\
\end{tabular}
\caption{Example specifications checked for each protocol. SMR protocols are configured to be $N$ fault-tolerant}
\label{tab:specifications}
\end{table*}



\begin{table}[tbh]
\centering
\scriptsize
\begin{tabular}{l|c|c|c}
%\hline
Protocols \ & Unhandled & \multicolumn{2}{c}{Spec. Violation}\\
\hhline{~~--}
Components & Event & Safety & Liveness\\\hline
Two Phase Commit & 20 & 15 & 4\\
Chain Repl. & 26 & 10 & 7\\
Multi-Paxos & 10 & 22 & 3\\
Basic Paxos & 6 & 6 & -\\
Leader Election & 9 & - & -\\
View Membership & 10 & 8 & 1\\
Fault Detector & 6 & 4 & - \\
\hline
%\hhline{=====}
\textbf{Total (167)}& 87 & 65 & 15\\
%\multicolumn{4}{c}{~}\\
%\multicolumn{4}{c}{\textit{Total bugs found = 167}}\\
%\hline
\end{tabular}
\caption{{\small Bugs found during development using compositional testing}}
\label{tab:bugsFound}
\end{table}


==> tex/intro_old.tex <==
\textbf{Link underutilization:}  They do no fully utilize the interconnects available on these machines. Link underutilized mainly refers to two aspects: homogeneous link underutilization, and heterogeneous link underutilization. First, for homogeneous links, 
given a topology, existed solutions do not always efficiently utilize all these available links.
This is because they all use ring-based protocols for data transfer and creates as many rings as possible with links available in the given topology.
%\footnote{Gloo has another option to use reduce-scatter borrowed from MPI domain, which needs a fully-connected network.}. 
In other words, they ignore the links that cannot form a new ring. 
Consider the topology in Figure \ref{fig:4gpu-broadcast}, representative of what can be found on modern NVIDIA DGX-1 servers~\cite{dgx1}, where we \textit{broadcast} from GPU A.
Since each link is bi-directional, there are two rings that we can construct as shown in Figure~\ref{fig:nccl4}.
Starting from A one ring is A->B->C->D->A, the other in reverse direction is A->C->D->B->A.
To broadcast, A can split data into two parts and send one part on each ring.
Thus if the data size is $n$ and link bandwidth size is $b$, the time taken will be $\frac{n}{2b}$.
Note that the two bidirectional, cross-bar links from A<->D and B<->C (shown as dashed lines) are not utilized! 
This link under-utilization issue becomes more severe in a shared/cloud environment, where partially allocated GPU group for each tenant forms irregular topology that causes more links being wasted.  


%\noindent\textbf{XXX: Say something about heterogeneity - different topologies, different types of interconnects (PCIe, NVLink, IB) and their characteristics.}

\textbf{Topology heterogeneity:} They stumble in achieving peak-performance in the face of every increasing hardware heterogeneity.  \textbf{XXX: Say something about (a) different typologies in DGX-1 based machines, (b) PCIe hierarchies (and highlight how current solutions limit themselves to homogeneous links), (c) dynamic assignment of resources by schedulers.}


\textbf{Link heterogeneity:} Existing schemes cannot effectively leverage different communication channels which may vary in bandwidth, topology, connected endpoints. State-of-the-art distributed Machine Learning (ML) platform may include links like 10Gbps Ethernet cables (1.25GB/s) and InfiniBand (6-7GB/s)~\cite{infiniband} for inter-node communication, PCIe (8-12GB/s)~\cite{pcie} and NVLink (20-25GB/s)~\cite{nvlink} for intra-node communication. Within a machine, PCIe connects CPU with multiple GPUs through PCIe switches in a tree hierarchy, whereas NVLink exists only among GPUs in a hyper-cube topology shown in Figure~\ref{fig:dgx1-topo}. Existing ring-based protocols fail to leverage link heterogeneity because they are assuming all the links in a ring have the same bit-rate. For example, for multi-GPU communication within a machine, NCCL only uses NVLink and ignores PCIe bus, due to the fact that PCIe link will be the bottleneck if it is included in a NVLink ring.

%PCIe is a shared bus used for intra-node, host-device communication, which has per-link (16-lane) top speed around 8-12GB/s. In a modern multi-GPU machine, PCIe bus forms a tree topology, where multiple GPUs are connected to a PCIe switch, which then connects to a CPU. Whereas NVLink is the interconnects only among GPUs within a machine, with maximum throughput between 20-25GB/s per each link \footnote{NVLink Gen1 in NVIDIA P100 GPU has max. throughput around 18-20GB/s, and NVLink Gen2 in NVIDIA V100 GPUs achieves 22-25GB/s.}. As shown in Figure ~\ref{fig:dgx1-topo}, NVLink topology is a hyper-cube structure linking 8GPUs. InfiniBand is used for cross-nodes communication at max speed around 6-7GB/s (HDR), which is multiple times higher than the commonly used 10Gbps Ethernet cables. 

To tackle these challenges, we propose {\tt \system{}}, a collectives communication library that achieves near-optimal link utilization regardless of link and topology heterogeneity. For topology heterogeneity, {\tt \system{}} automatically adapt to new inter-connect topologies (especially for the irregular topology due to partial allocated GPU group) and provide optional solutions. For link heterogeneity, {\tt \system{}} achieves hybrid data transfer over heterogeneous links simultaneously (PCIe, NVLink, InifiniBand). From the programmer perspective, {\tt \system{}} provides NCCL-compatible API, so that there is no need of user-level code changes and {\tt \system{}} can be naturally plugged into distributed ML framework like TensorFlow~\cite{tensorflow}, PyTorch~\cite{pytorch}, CNTK~\cite{cntk}, MxNet~\cite{mxnet}, etc.


Achieving optimal throughput over varies kinds of topology is non-trivial because (1) each round of collective communication needs to reach to all GPUs in use. (2) The most frequently-used primitive (i.e. All-Reduce) may need to involve two round of communication, one round for computation like add or average, the second round is for broadcast the final aggregated result. And \emph{ring} is the simplest way to tackle these two challenges. 


For the first challenge, it is obvious for ring-based solutions since all the nodes are connected in a ring. 
But ring-based solutions are under strong assumptions that: for each ring, (a) each node can only have 1 input link and 1 output link, (b) the picked links connecting all the nodes must form a circle. These two assumptions leads to link under-utilization because it excludes the cases like: nodes may have different number of input degree and output degree, which may not be equal to 1. The picked links for completing one collective communication process may have a spanning tree topology, ring is just a speical subset of spanning tree. Based on these observations, {\tt \system{}} breaks the ring to adopt the cases that ring cannot support. At the high level, {\tt \system{}} leverages all available links by packing as many spanning trees as possible into the topology. Accordingly, we create collective primitives that only needs one round communication (e.g. broadcast, gather, reduce). One thing worth mentioning is that, in order to create a ring, we need \# of GPU links, but to create a spanning tree, we need (\# of GPU - 1) links which saves 1 link for further link allocation.


For the second challenge, ring-based solutions can easily handle it by aggregating each node's local data into the partially added/averaged global data which is received from predecessor, and the pass it to its successor. Since the communication channel forms a loop, no matter which node (as the root) start the collective communication, they can always finish it by passing data in one direction. And it takes two rounds over the ring, the first round to get the final result on the predecessor before the starting node, the second round is to broadcast the final result through the nodes in the ring. However, it is not the case for {\tt \system{}}'s spanning tree structure. We can easily finish the first round data aggregation in the reverse direction of a spanning tree. However, except the root node, other nodes cannot get the final result since there is no loop-back link to achieve similar broadcast round in ring-based solutions. And we cannot randomly pick another spanning tree with a different root node to mimic the 2nd round broadcast in ring-based solution, due to the fact that the picked root node may not have the final aggregated result. Furthermore, even we pick another spanning tree start from the node that has the final aggregated result, it may still not be link-efficient, since the new tree may have conflict links with the original tree, which decrease the throughput. To address this issue, we leverage the bi-directional attribute of the link we use, and propose an alternative design in {\tt \system{}}. Basically, given a spanning tree, we first do reduce in the reverse direction of the spanning tree, and then broadcast the aggregated result from the root node in the spanning tree.

\gw{tiny contribution, maybe not put it here} We also introduce a number of techniques to improve performance. In ring, each node only needs to hold 1 input buffer and 1 output buffer. To match the NCCL API (which only passing in 1 input and 1 output buffer addresses), and also reduce overhead of creating multiple input/output buffers, we use Unified Virtual Addressing (UVA), instead of buffering the input data on the destination GPU, we directly pull the data from source GPU/s when it is needed.

To leverage link heterogeneity, {\tt \system{}} adopt hybrid data transfer over PCIe and NVLink within a machine, and use IB for inter-node communication. Basically, we use PCIe hierarchy to create one ring for collective communication, at the same time, create multiple spanning tree over NVLinks. How to determine the data split between PCIe ring and NVLink spanning trees is a problem. To find the optimal solution, before real collective communication happen, we need to do some test runs which collects information like PCIe topology, PCIe bandwidth, NVLink topology, NVLink bandwidth etc. And based on these information, we design a function to automatically provide the optimal data split between NVLink and PCIe channels. For inter-node communication using IB, we also designed a pipeline scheme which can fully utilize IB bandwidth to achieve decent performance.

In summary, we make the following contributions:
\begin{itemize}
\item We breaks the ring, and adopt a more general spanning tree scheme, which achieve better link utilization.
\item We leverage the bi-direction attribute of the link to finish two rounds collective communication like all-reduce within one spanning tree.
\item We leverage link heterogeneity to achieve hybrid collective communication over PCIe ring and NVLink spanning trees within a machine, and use IB for cross-machine communication.
\end{itemize}

{\tt \system{}} Performacen highlight: compare with NCCL, we have 2-6x speed up

\amar{Need to fix intro!}

\begin{itemize}
\item motivation - why do we think we can do better?  high-level design. (Section~\ref{sec:motivation})
\item detail the hardware capabilities of modern GPU accelerators with an emphasis on compute and interconnect capabilities (Section~\ref{sec:ubench}).
\item how do we do better?  given gpu allocation and annotated topology information, optimizer spits out transfer schedule.  tie in to microbenchmarks. (Section~\ref{sec:design}).
\item experiments - ubench and end-to-end.  (Section~\ref{sec:eval}).
\item related work (Section~\ref{sec:related}).
\item conclusion (Section~\ref{sec:concl}).
\end{itemize}


